Monotone level-sets on arbitrary meshes without redistancing

In this paper we present approaches that address two issues that can occur when the level-set method is used to simulate two-fluid flows in engineering practice. The first issue concerns regularizing the Heaviside function on arbitrary meshes. We show that the regularized Heaviside function can be non-smooth on non-uniform meshes. Alternative regularizing definitions that are indeed smooth and monotonic, are introduced. These new definitions lead to smooth Heaviside functions by taking the changing local meshsize into account. The second issue is the computational cost and fragility caused by the necessity of redistancing the level-set field. In previous papers it is shown that strongly coupling the level-set convection with the flow solver provides robustness and potentially efficiency and accuracy advantages. The next step would be to include redistancing within the strong coupling part of the algorithm. The computational cost of current redistancing procedure prohibit this. Four alternative approaches for circumventing the expensive redistancing step are proposed. This should facilitate a fully coupled level-set approach. Some benchmark cases demonstrate the efficacy of the proposed approaches. These includes the standard test case of the vortex in a box. Based on these results the most favorable redistancing approach is selected.

==> conv.tex <==
\relax 


==> conv/L1_H_2.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(826,590)(0,0)
\font\gnuplot=cmr10 at 7pt
\gnuplot
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(134.0,92.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,92.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,119.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,119.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,141.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,141.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,159.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,159.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,175.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,175.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,189.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,189.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,202.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(120,202){\makebox(0,0)[r]{ 0.01}}
\put(763.0,202.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(134.0,285.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,285.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,334.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,334.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,368.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,368.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,395.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,395.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,417.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,417.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,435.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,435.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,451.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,451.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,465.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,465.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,478.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(120,478){\makebox(0,0)[r]{ 0.1}}
\put(763.0,478.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(134.0,561.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,561.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(134,63){\makebox(0,0){ 0.01}}
\put(134.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(325.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(325,63){\makebox(0,0){ 0.02}}
\put(325.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(437.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(437,63){\makebox(0,0){ 0.03}}
\put(437.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(517.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(517,63){\makebox(0,0){ 0.04}}
\put(517.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(578.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(578,63){\makebox(0,0){ 0.05}}
\put(578.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(671.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(671,63){\makebox(0,0){ 0.07}}
\put(671.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(770.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(770,63){\makebox(0,0){ 0.1}}
\put(770.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(134.0,92.0){\rule[-0.200pt]{0.400pt}{112.982pt}}
\put(134.0,92.0){\rule[-0.200pt]{156.344pt}{0.400pt}}
\put(783.0,92.0){\rule[-0.200pt]{0.400pt}{112.982pt}}
\put(134.0,561.0){\rule[-0.200pt]{156.344pt}{0.400pt}}
\put(21,326){\makebox(0,0){\rotatebox{90}{$L_1(H)$}}}
\put(458,20){\makebox(0,0){$h$}}
\put(665,185){\makebox(0,0)[r]{$C_0-P_1$}}
\put(679.0,185.0){\rule[-0.200pt]{18.308pt}{0.400pt}}
\put(770,506){\usebox{\plotpoint}}
\multiput(754.40,504.92)(-4.642,-0.496){39}{\rule{3.757pt}{0.119pt}}
\multiput(762.20,505.17)(-184.202,-21.000){2}{\rule{1.879pt}{0.400pt}}
\multiput(571.60,483.92)(-1.810,-0.498){103}{\rule{1.542pt}{0.120pt}}
\multiput(574.80,484.17)(-187.801,-53.000){2}{\rule{0.771pt}{0.400pt}}
\multiput(383.10,430.92)(-1.051,-0.499){179}{\rule{0.940pt}{0.120pt}}
\multiput(385.05,431.17)(-189.050,-91.000){2}{\rule{0.470pt}{0.400pt}}
\put(770,506){\makebox(0,0){$+$}}
\put(578,485){\makebox(0,0){$+$}}
\put(387,432){\makebox(0,0){$+$}}
\put(196,341){\makebox(0,0){$+$}}
\put(717,185){\makebox(0,0){$+$}}
\put(665,156){\makebox(0,0)[r]{$C_0-Q_1$}}
\multiput(679,156)(20.756,0.000){4}{\usebox{\plotpoint}}
\put(755,156){\usebox{\plotpoint}}
\put(770,513){\usebox{\plotpoint}}
\multiput(770,513)(-20.490,-3.308){10}{\usebox{\plotpoint}}
\multiput(578,482)(-19.180,-7.933){10}{\usebox{\plotpoint}}
\multiput(387,403)(-18.776,-8.847){10}{\usebox{\plotpoint}}
\put(196,313){\usebox{\plotpoint}}
\put(770,513){\makebox(0,0){$\times$}}
\put(578,482){\makebox(0,0){$\times$}}
\put(387,403){\makebox(0,0){$\times$}}
\put(196,313){\makebox(0,0){$\times$}}
\put(717,156){\makebox(0,0){$\times$}}
\sbox{\plotpoint}{\rule[-0.400pt]{0.800pt}{0.800pt}}%
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(665,127){\makebox(0,0)[r]{$C_1-Q_2$}}
\sbox{\plotpoint}{\rule[-0.400pt]{0.800pt}{0.800pt}}%
\put(679.0,127.0){\rule[-0.400pt]{18.308pt}{0.800pt}}
\put(770,506){\usebox{\plotpoint}}
\multiput(761.76,504.09)(-1.120,-0.501){165}{\rule{1.986pt}{0.121pt}}
\multiput(765.88,504.34)(-187.878,-86.000){2}{\rule{0.993pt}{0.800pt}}
\multiput(572.70,418.09)(-0.673,-0.501){277}{\rule{1.276pt}{0.121pt}}
\multiput(575.35,418.34)(-188.351,-142.000){2}{\rule{0.638pt}{0.800pt}}
\multiput(380.46,276.09)(-0.862,-0.501){215}{\rule{1.577pt}{0.121pt}}
\multiput(383.73,276.34)(-187.728,-111.000){2}{\rule{0.788pt}{0.800pt}}
\put(770,506){\makebox(0,0){$\ast$}}
\put(578,420){\makebox(0,0){$\ast$}}
\put(387,278){\makebox(0,0){$\ast$}}
\put(196,167){\makebox(0,0){$\ast$}}
\put(717,127){\makebox(0,0){$\ast$}}
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(134.0,92.0){\rule[-0.200pt]{0.400pt}{112.982pt}}
\put(134.0,92.0){\rule[-0.200pt]{156.344pt}{0.400pt}}
\put(783.0,92.0){\rule[-0.200pt]{0.400pt}{112.982pt}}
\put(134.0,561.0){\rule[-0.200pt]{156.344pt}{0.400pt}}
\end{picture}


==> conv/Linf_phi_2.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\begin{picture}(826,590)(0,0)
\font\gnuplot=cmr10 at 7pt
\gnuplot
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(134.0,92.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(120,92){\makebox(0,0)[r]{ 0.01}}
\put(763.0,92.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(134.0,180.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,180.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,232.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,232.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,268.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,268.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,297.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,297.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,320.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,320.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,339.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,339.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,356.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,356.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,371.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,371.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,385.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(120,385){\makebox(0,0)[r]{ 0.1}}
\put(763.0,385.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(134.0,473.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,473.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,524.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,524.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,561.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(773.0,561.0){\rule[-0.200pt]{2.409pt}{0.400pt}}
\put(134.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(134,63){\makebox(0,0){ 0.01}}
\put(134.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(325.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(325,63){\makebox(0,0){ 0.02}}
\put(325.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(437.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(437,63){\makebox(0,0){ 0.03}}
\put(437.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(517.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(517,63){\makebox(0,0){ 0.04}}
\put(517.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(578.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(578,63){\makebox(0,0){ 0.05}}
\put(578.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(671.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(671,63){\makebox(0,0){ 0.07}}
\put(671.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(770.0,92.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(770,63){\makebox(0,0){ 0.1}}
\put(770.0,541.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(134.0,92.0){\rule[-0.200pt]{0.400pt}{112.982pt}}
\put(134.0,92.0){\rule[-0.200pt]{156.344pt}{0.400pt}}
\put(783.0,92.0){\rule[-0.200pt]{0.400pt}{112.982pt}}
\put(134.0,561.0){\rule[-0.200pt]{156.344pt}{0.400pt}}
\put(21,326){\makebox(0,0){\rotatebox{90}{$L_{\infty}(\phi)$}}}
\put(458,20){\makebox(0,0){$h$}}
\put(665,185){\makebox(0,0)[r]{$C_0-P_1$}}
\put(679.0,185.0){\rule[-0.200pt]{18.308pt}{0.400pt}}
\put(770,542){\usebox{\plotpoint}}
\multiput(761.41,540.92)(-2.479,-0.498){75}{\rule{2.069pt}{0.120pt}}
\multiput(765.71,541.17)(-187.705,-39.000){2}{\rule{1.035pt}{0.400pt}}
\multiput(573.24,501.92)(-1.312,-0.499){143}{\rule{1.147pt}{0.120pt}}
\multiput(575.62,502.17)(-188.620,-73.000){2}{\rule{0.573pt}{0.400pt}}
\multiput(382.30,428.92)(-1.294,-0.499){145}{\rule{1.132pt}{0.120pt}}
\multiput(384.65,429.17)(-188.650,-74.000){2}{\rule{0.566pt}{0.400pt}}
\put(770,542){\makebox(0,0){$+$}}
\put(578,503){\makebox(0,0){$+$}}
\put(387,430){\makebox(0,0){$+$}}
\put(196,356){\makebox(0,0){$+$}}
\put(717,185){\makebox(0,0){$+$}}
\put(665,156){\makebox(0,0)[r]{$C_0-Q_1$}}
\multiput(679,156)(20.756,0.000){4}{\usebox{\plotpoint}}
\put(755,156){\usebox{\plotpoint}}
\put(770,557){\usebox{\plotpoint}}
\multiput(770,557)(-19.721,-6.471){10}{\usebox{\plotpoint}}
\multiput(578,494)(-18.926,-8.521){10}{\usebox{\plotpoint}}
\multiput(387,408)(-19.319,-7.586){10}{\usebox{\plotpoint}}
\put(196,333){\usebox{\plotpoint}}
\put(770,557){\makebox(0,0){$\times$}}
\put(578,494){\makebox(0,0){$\times$}}
\put(387,408){\makebox(0,0){$\times$}}
\put(196,333){\makebox(0,0){$\times$}}
\put(717,156){\makebox(0,0){$\times$}}
\sbox{\plotpoint}{\rule[-0.400pt]{0.800pt}{0.800pt}}%
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(665,127){\makebox(0,0)[r]{$C_1-Q_2$}}
\sbox{\plotpoint}{\rule[-0.400pt]{0.800pt}{0.800pt}}%
\put(679.0,127.0){\rule[-0.400pt]{18.308pt}{0.800pt}}
\put(770,527){\usebox{\plotpoint}}
\multiput(762.24,525.09)(-1.047,-0.501){177}{\rule{1.870pt}{0.121pt}}
\multiput(766.12,525.34)(-188.120,-92.000){2}{\rule{0.935pt}{0.800pt}}
\multiput(572.21,433.09)(-0.747,-0.501){249}{\rule{1.394pt}{0.121pt}}
\multiput(575.11,433.34)(-188.107,-128.000){2}{\rule{0.697pt}{0.800pt}}
\multiput(381.70,305.09)(-0.673,-0.501){277}{\rule{1.276pt}{0.121pt}}
\multiput(384.35,305.34)(-188.351,-142.000){2}{\rule{0.638pt}{0.800pt}}
\put(770,527){\makebox(0,0){$\ast$}}
\put(578,435){\makebox(0,0){$\ast$}}
\put(387,307){\makebox(0,0){$\ast$}}
\put(196,165){\makebox(0,0){$\ast$}}
\put(717,127){\makebox(0,0){$\ast$}}
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(134.0,92.0){\rule[-0.200pt]{0.400pt}{112.982pt}}
\put(134.0,92.0){\rule[-0.200pt]{156.344pt}{0.400pt}}
\put(783.0,92.0){\rule[-0.200pt]{0.400pt}{112.982pt}}
\put(134.0,561.0){\rule[-0.200pt]{156.344pt}{0.400pt}}
\end{picture}


==> smooth/notics/arb1_mesh.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\begin{picture}(826,118)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(50,78){\usebox{\plotpoint}}
\put(50,78){\makebox(0,0){$+$}}
\put(178,78){\makebox(0,0){$+$}}
\put(178,78){\makebox(0,0){$+$}}
\put(273,78){\makebox(0,0){$+$}}
\put(273,78){\makebox(0,0){$+$}}
\put(337,78){\makebox(0,0){$+$}}
\put(337,78){\makebox(0,0){$+$}}
\put(379,78){\makebox(0,0){$+$}}
\put(379,78){\makebox(0,0){$+$}}
\put(408,78){\makebox(0,0){$+$}}
\put(408,78){\makebox(0,0){$+$}}
\put(436,78){\makebox(0,0){$+$}}
\put(436,78){\makebox(0,0){$+$}}
\put(478,78){\makebox(0,0){$+$}}
\put(478,78){\makebox(0,0){$+$}}
\put(542,78){\makebox(0,0){$+$}}
\put(542,78){\makebox(0,0){$+$}}
\put(637,78){\makebox(0,0){$+$}}
\put(637,78){\makebox(0,0){$+$}}
\put(765,78){\makebox(0,0){$+$}}
\put(50.0,78.0){\rule[-0.200pt]{172.243pt}{0.400pt}}
\put(50,40){\usebox{\plotpoint}}
\put(50.00,40.00){\usebox{\plotpoint}}
\put(70.76,40.00){\usebox{\plotpoint}}
\put(91.51,40.00){\usebox{\plotpoint}}
\put(112.27,40.00){\usebox{\plotpoint}}
\put(133.02,40.00){\usebox{\plotpoint}}
\put(153.78,40.00){\usebox{\plotpoint}}
\put(174.53,40.00){\usebox{\plotpoint}}
\put(195.29,40.00){\usebox{\plotpoint}}
\put(216.04,40.00){\usebox{\plotpoint}}
\put(236.80,40.00){\usebox{\plotpoint}}
\put(257.56,40.00){\usebox{\plotpoint}}
\put(278.31,40.00){\usebox{\plotpoint}}
\put(299.07,40.00){\usebox{\plotpoint}}
\put(319.82,40.00){\usebox{\plotpoint}}
\put(340.58,40.00){\usebox{\plotpoint}}
\put(361.33,40.00){\usebox{\plotpoint}}
\put(382.09,40.00){\usebox{\plotpoint}}
\put(402.84,40.00){\usebox{\plotpoint}}
\put(423.60,40.00){\usebox{\plotpoint}}
\put(444.35,40.00){\usebox{\plotpoint}}
\put(465.11,40.00){\usebox{\plotpoint}}
\put(485.87,40.00){\usebox{\plotpoint}}
\put(506.62,40.00){\usebox{\plotpoint}}
\put(527.38,40.00){\usebox{\plotpoint}}
\put(548.13,40.00){\usebox{\plotpoint}}
\put(568.89,40.00){\usebox{\plotpoint}}
\put(589.64,40.00){\usebox{\plotpoint}}
\put(610.40,40.00){\usebox{\plotpoint}}
\put(631.15,40.00){\usebox{\plotpoint}}
\put(651.91,40.00){\usebox{\plotpoint}}
\put(672.66,40.00){\usebox{\plotpoint}}
\put(693.42,40.00){\usebox{\plotpoint}}
\put(714.18,40.00){\usebox{\plotpoint}}
\put(734.93,40.00){\usebox{\plotpoint}}
\put(755.69,40.00){\usebox{\plotpoint}}
\put(765,40){\usebox{\plotpoint}}
\end{picture}


==> smooth/notics/uni_mesh.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(826,118)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(50,78){\usebox{\plotpoint}}
\put(50,78){\makebox(0,0){$+$}}
\put(121,78){\makebox(0,0){$+$}}
\put(121,78){\makebox(0,0){$+$}}
\put(193,78){\makebox(0,0){$+$}}
\put(193,78){\makebox(0,0){$+$}}
\put(265,78){\makebox(0,0){$+$}}
\put(265,78){\makebox(0,0){$+$}}
\put(336,78){\makebox(0,0){$+$}}
\put(336,78){\makebox(0,0){$+$}}
\put(408,78){\makebox(0,0){$+$}}
\put(408,78){\makebox(0,0){$+$}}
\put(479,78){\makebox(0,0){$+$}}
\put(479,78){\makebox(0,0){$+$}}
\put(551,78){\makebox(0,0){$+$}}
\put(551,78){\makebox(0,0){$+$}}
\put(622,78){\makebox(0,0){$+$}}
\put(622,78){\makebox(0,0){$+$}}
\put(694,78){\makebox(0,0){$+$}}
\put(694,78){\makebox(0,0){$+$}}
\put(765,78){\makebox(0,0){$+$}}
\put(50.0,78.0){\rule[-0.200pt]{172.243pt}{0.400pt}}
\put(50,40){\usebox{\plotpoint}}
\put(50.00,40.00){\usebox{\plotpoint}}
\put(70.76,40.00){\usebox{\plotpoint}}
\put(91.51,40.00){\usebox{\plotpoint}}
\put(112.27,40.00){\usebox{\plotpoint}}
\put(133.02,40.00){\usebox{\plotpoint}}
\put(153.78,40.00){\usebox{\plotpoint}}
\put(174.53,40.00){\usebox{\plotpoint}}
\put(195.29,40.00){\usebox{\plotpoint}}
\put(216.04,40.00){\usebox{\plotpoint}}
\put(236.80,40.00){\usebox{\plotpoint}}
\put(257.56,40.00){\usebox{\plotpoint}}
\put(278.31,40.00){\usebox{\plotpoint}}
\put(299.07,40.00){\usebox{\plotpoint}}
\put(319.82,40.00){\usebox{\plotpoint}}
\put(340.58,40.00){\usebox{\plotpoint}}
\put(361.33,40.00){\usebox{\plotpoint}}
\put(382.09,40.00){\usebox{\plotpoint}}
\put(402.84,40.00){\usebox{\plotpoint}}
\put(423.60,40.00){\usebox{\plotpoint}}
\put(444.35,40.00){\usebox{\plotpoint}}
\put(465.11,40.00){\usebox{\plotpoint}}
\put(485.87,40.00){\usebox{\plotpoint}}
\put(506.62,40.00){\usebox{\plotpoint}}
\put(527.38,40.00){\usebox{\plotpoint}}
\put(548.13,40.00){\usebox{\plotpoint}}
\put(568.89,40.00){\usebox{\plotpoint}}
\put(589.64,40.00){\usebox{\plotpoint}}
\put(610.40,40.00){\usebox{\plotpoint}}
\put(631.15,40.00){\usebox{\plotpoint}}
\put(651.91,40.00){\usebox{\plotpoint}}
\put(672.66,40.00){\usebox{\plotpoint}}
\put(693.42,40.00){\usebox{\plotpoint}}
\put(714.18,40.00){\usebox{\plotpoint}}
\put(734.93,40.00){\usebox{\plotpoint}}
\put(755.69,40.00){\usebox{\plotpoint}}
\put(765,40){\usebox{\plotpoint}}
\end{picture}

